Multi-Fact Correction in Abstractive Text Summarization

Pre-trained neural abstractive summarization systems have dominated extractive strategies on news summarization performance, at least in terms of ROUGE. However, system-generated abstractive summaries often face the pitfall of factual inconsistency: generating incorrect facts with respect to the source text. To address this challenge, we propose Span-Fact, a suite of two factual correction models that leverages knowledge learned from question answering models to make corrections in system-generated summaries via span selection. Our models employ single or multi-masking strategies to either iteratively or auto-regressively replace entities in order to ensure semantic consistency w.r.t. the source text, while retaining the syntactic structure of summaries generated by abstractive summarization models. Experiments show that our models significantly boost the factual consistency of system-generated summaries without sacrificing summary quality in terms of both automatic metrics and human evaluation.

==> legacy/5_dataset_quality.tex <==
\section{Dataset Quality Analysis}
% \subsection{Is Abstract information sufficient for relation work?}
% Randomly select 50-100 samples from test set to perform human evaluation

% 4 (perfect reconstruct): 75\% - 100\% 

% 3 (include major facts): 50\% - 75\% content can be reconstructed

% 2 (include partial facts): 25\% - 50\% content can be reconstructed

% 1 (almost no facts): 0\% - 25\% content can be reconstructed

% \subsection{The clustering of content information: All in CS}

\subsection{Abstractive or Extractive?}
\yaolu{Table: Ranking of models output in terms of generation quality}. It is obvious that due to the writing style of related work, the abstractive model consistently outperformed extractive model in terms of human quality ranking.




==> legacy/z2_related_work.tex <==


% \section{Related Work}
% \begin{itemize}
%     \item news-based summ (single \& multi), DUC, CNNDM, NYT XSUM
%     \item wiki summarization: wikisumm 
%   \item academic summ (scisumm- the workshop, tldr-allenai?, \cite{yasunaga2019scisummnet} small evaluation set) academic single summ (arxiv \& pubmed)
%     t\item extreme summ(tldr-allenai, small size,   XSUM- single version)

% \end{itemize}




% There are multiple \cite{Radev&al.13, Radev&al.09, Radev&al.09a}
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c}\toprule

%         dd    &      SINGLE          & MULTI    \toprule

% NEWS        &     CNNDM.NYT.XSUM  & Multi-News \hline
% WIKI        &     -               & WIKISUM \hline
% SCIENCE     &     ARXIV/PUBMED    & Multi-Science(ours)\hline 

%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}



==> motivation.tex <==
%In this section, we describe motivation of focus on entity correction based on the QA module in Section \ref{subsec:model_fact_error_analysis}. We then describe the two models we proposed for factual error correction based on QA modules. 

% \subsection{Error analysis on factual errors in factCC}
% \label{subsec:model_fact_error_analysis}
% \begin{table}[h!]
% \centering
% \resizebox{\columnwidth}{!}{%
% %   \begin{center}{\footnotesize
%   \begin{tabular}{ l | c c c c } %  l l l l | l l l | l l l}
%     \toprule
%      \multirow{2}{*}{Datasets} & \multicolumn{4}{c}{\% of error types} \\
%     & number entities & name entities & xx-entities & \# other \\ \toprule
%     factCC & - & - & - & - \\

%     CNNDM & - & - & - & - \\
%     XSUM & - & - & - & - \\
   
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{\small ).}\label{table:error_type_analysis}
% \end{table}

% Table \ref{table:error_type_analysis} provides our human evaluation on the error type analysis of examples that factCC models identity as incorrect for various summarization systems. We annotate the error types of the summaries, and found XX percent among them are entity errors. Especially, We found on XSum, the model is hallucinating significantly, which verifies the claim of \citet{maynez2020faithfulness} that this dataset is more abstractive and current abstractive summarization models are struggling to make the entities correct on the summary. This observation motivate us to deal with entity correction specifically in this project. 
